In-Context Editing: Learning Knowledge from Self-Induced Distributions

In scenarios where language models must incorporate new information efficiently without extensive retraining, traditional fine-tuning methods are prone to overfitting, degraded generalization, and unnatural language generation. To address these limitations, we introduce Consistent In-Context Editing (ICE), a novel approach leveraging the model's in-context learning capability to optimize toward a contextual distribution rather than a one-hot target. ICE introduces a simple yet effective optimization framework for the model to internalize new knowledge by aligning its output distributions with and without additional context. This method enhances the robustness and effectiveness of gradient-based tuning methods, preventing overfitting and preserving the model's integrity. We analyze ICE across four critical aspects of knowledge editing: accuracy, locality, generalization, and linguistic quality, demonstrating its advantages. Experimental results confirm the effectiveness of ICE and demonstrate its potential for continual editing, ensuring that the integrity of the model is preserved while updating information.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/analysis.tex <==
\section{Analysis}
\label{sec:analysis}
\subsection{Accuracy and Linguistic Quality}
The proposed \autoref{alg:ice} effectively maximizes the likelihood of sampled sequences conditioned on the target tokens. After mathematical manipulations (\autoref{appendix:sec:decompose_ice}), the overall optimization objective is equivalent to a combination of two losses:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{ft} + \mathcal{L}_{ice}\Bigl([\vq,\mathbf{x}^*]\Bigr),
\end{equation}
where the second term is the consistent in-context editing loss $\mathcal{L}_{ice}$ with the substitution $\vq \leftarrow [\vq,\mathbf{x}^*]$. 

The \textbf{accuracy} of our method is ensured by the first term $\mathcal{L}_{ft}$. This guides the model to maximize both $p_{\theta}(\vx^* | \vq)$ and $p_{\theta}(\vx^{*} | [\vc, \vq])$ throughout the optimization process, effectively aligning with the target $\vx^*$ as it becomes the most probable output.

The \textbf{linguistic quality} is maintained by $\mathcal{L}_{ice}\Bigl([\vq,\mathbf{x}^*]\Bigr)$, which fits the model on a self-induced distribution rather than overfitting on a single target. By using the context to guide the model, we create a broader, more representative distribution that preserves the natural variability and richness of language, thereby avoiding repetitive or incoherent outputs and ensuring high-quality and contextually appropriate language generation.

\subsection{Locality and Generalization}
To understand how the proposed method maintains locality and potentially improves generalization, we divide all possible query-response pairs into two sets: $(\vq, \vx) \in \mathcal{D}_q \cup \mathcal{D}_{\neg q}$, where $\mathcal{D}_{\neg q}$ is the complement of the set $\mathcal{D}_q$ related to the target knowledge. The in-context editing loss term can be decomposed as follows:
\begin{equation}
\scalebox{0.9}{$
\begin{aligned}
\mathcal{L}_{ice} &= D_{KL}( p_{\theta}(\vx | [\vc, \vq]) \;||\; p_{\theta}(\vx | \vq)) \\
&= \sum_{(\vq, \vx) \sim \mathcal{D}_q \cup \mathcal{D}_{\neg q}} p_{\theta}(\vx | [\vc, \vq]) \log\left(\frac{ p_{\theta}(\vx | [\vc, \vq])}{p_{\theta}(\vx | \vq)}\right).
\end{aligned}
$}
\end{equation}
Hence \textbf{locality} is ensured by the loss on the set $\mathcal{D}_{\neg q}$, as $p_{\theta}(\vx | [\vc, \vq])$ should maintain the original responses when the context $\vc$ is unrelated to the query $\vq$. On the other hand, the loss on the set $\mathcal{D}_q$ introduces \textbf{generalization}, provided that the model's in-context capability is strong enough to extend the knowledge provided in $\vc$ to answer related queries $\vq$. Thus the effectiveness of this strategy relies on the following assumptions:

\textit{The context is related to the knowledge}. The context provided in the prompts must be pertinent and relevant to the knowledge needed for generating accurate and coherent responses. This relevance ensures that the additional information introduced through the context is meaningful and enhances the model's understanding of the query.
    
\textit{The model attends to the context}. The model must be capable of attending to and incorporating the contextual information provided in the prompts. During the fine-tuning process, the model effectively uses the context as part of its input, influencing its predictions and overall performance.
    
\textit{The model generalizes from the context to related knowledge}. Given the relevant context, the model should be able to generalize from the specific information in the context to broader or related knowledge areas. This generalization enables the model to generate responses that are not only contextually coherent but also enriched with additional details inferred from the context. Techniques like chain-of-thought ~\cite{wei2022chain} can potentially be employed in the context prompt to enhance the model's generalization capability.

==> sections/backup/analysis_backup.tex <==
\section{Analysis}
\subsection{Fine-tuning with Sampling}
Current methodologies for model fine-tuning frequently employ a one-hot distribution based on a single example $(\vq^*, \vx^*)$. The fine-tuning objective, in this context, is the Kullback-Leibler (KL) divergence between the one-hot distribution $\mathbbm{1}(x_{1:m}; \mathbf{x}^*)$ and the model's predicted distribution $p_\theta(x_{1:m}| \vq^*)$\,. This objective can be defined as follows:
\begin{equation}
	L_{ft} \equiv KL\left[\mathbbm{1}(x_{1:m}; \vx^*) \| p_\theta(x_{1:m}| \vq^*)\right],
	\label{eq:ft}
\end{equation}
where $\mathbbm{1}(x_{1:m}; \vx^*)$ is the one-hot distribution which is more formally given by:
\[
\mathbbm{1}(\vx; \vy) \equiv \prod_i \delta(x_i, y_i),
\]
with
\[
\delta(x_i, y_i) \equiv
	\begin{cases}
	  1 & \text{if } x_i = y_i \\
	  0 & \text{if } x_i \neq y_i
	\end{cases}.
\]
The fine-tuning loss $L_{ft}$ given in ~\autoref{eq:ft} can be simplified to:
\begin{equation}
	L_{ft} = - \log p_\theta(\vx^* | \vq^*),
\end{equation}
which aligns with the maximum likelihood estimation (MLE) objective.

For fine tuning with sampling, objective $L^*_{ft}$ is expressed as:
\begin{align}
		L^*_{ft} \equiv KL&[\mathbbm{1}(x_{1:m}; \vx^*)p_\theta\left(\left. x_{m+1:T}\right|\left[\vq^*, \vx^*\right]\right) \nonumber\\
  &\|\;p_\theta\left(x_{1:T}|\vq^*\right)]
	\label{eq:self_finetune}
\end{align}
where $x_{1:T}$ is the sequence truncated at length $T$.


\subsection{In-context Fine Tuning}
The objective $L_{icft}$ aims to minimize the KL divergence between the model's in-context distribution and its original predicted distribution:
\begin{equation}
	L_{icft}(\vq)\equiv KL\left[p_\theta\bigl(x_{1:T}|[\vc,\vq^*]\bigr)\|p_\theta(x_{1:T}|\vq^*)\right].
\end{equation}
Compared to direct fine-tuning, the efficacy of in-context fine-tuning depends on both the quality of the context and the model's ability to utilize the provided context. Thus, the effectiveness of this strategy relies on the following assumptions:
\begin{enumerate}
    \item \textbf{Context is related to the knowledge:} It is assumed that the context provided in the prompts is pertinent and relevant to the knowledge needed for generating accurate and coherent responses. This relevance ensures that the additional information introduced through the context is meaningful and enhances the model's understanding of the query.
    
    \item \textbf{The model attends to the context:} The model has the capability to attend to and incorporate the contextual information provided in the prompts. This means that during the fine-tuning process, the model effectively uses the context as part of its input, influencing its predictions and overall performance.
    
    \item \textbf{The model generalizes from the context to related knowledge:} Given the relevant context, the model is capable of generalizing from the specific information in the context to broader or related knowledge areas. This generalization allows the model to generate responses that are not only contextually coherent but also enriched with additional details inferred from the context.
\end{enumerate}

{\color{blue}
Divided into in-scope set and out-of-scope set.


\begin{prop}
Sampling with contexts preserves locality.
\end{prop}


\begin{prop}
Sampling with contexts generalizes.
\end{prop}

Potentially combine with CoT techniques to improve generalization.
}

\subsection{Consistent In-context Fine Tuning}
\textcolor{blue}{
However, the target is not necessarily correct, \ie, adding contexts does not guarantee the \textbf{accuracy} of the model. Hence dynamic training target.\\
Consistency model:
Equations.\\
This pulls the distribution to satisfy the constraint.\\
A hypothesis is that it does instruction tuning + finetuning at the same time.}

Formally, the objective of consistent in-context fine tuning can be expressed as:
\begin{align*}
	L^{*}_{icft}  =
	KL[&\mathbbm{1}(x_{1:m}; \vx^*)\;p_\theta\left(\left. x_{m+1:\infty}\right|\left[\vc,\vq, \vx^*\right]\right) \\
    &\| p_\theta\left(x_{1:\infty}|\vq\right)] 
\end{align*}
where the target distribution incorporates the one-hot encoding of the target sequence $\vx^*$ as part of the input, effectively "pulling" the model's predicted distribution towards generating the correct sequence. 

After mathematical manipulations, we can express the overall loss function as:

\begin{equation*}
    L^{*}_{icft}  = L_{ft}+ L_{icft}\Bigl([\vq,\mathbf{x}^*]\Bigr),
\end{equation*}
where the second term is equivalent to the in-context fine-tuning loss $L_{icft}$ with the replacements $\vq \rightarrow [\vq,\mathbf{x}^*]$.

This consistency model effectively "pulls the distribution" towards the desired target sequence $\vx^*$ by incorporating $L_{ft}$ directly into the ICFT loss $L_{icft}$. This combined approach aims to satisfy the accuracy constraint while maintaining the benefits of locality and generalization achieved through the use of context prompts.

A key hypothesis is that this dynamic training target, which integrates instruction tuning and fine-tuning simultaneously, can further improve the language model's performance in the knowledge editing task, addressing the limitations of the previous approach and ensuring both accuracy and coherence in the model's responses.

==> sections/backup/exp_backup.tex <==
\begin{table}[t]
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\textbf{DataSet} & \textbf{Metric} & \textbf{ROME} & \textbf{MEMIT} & \textbf{FT-L} & \textbf{FT-M} & \textbf{ICE} \\
\midrule
\multirow{5}{*}{\textbf{Wiki$_{recent}$}} & Edit Succ. $\uparrow$ & 97.25 & 97.03 & 45.63 & 100.00 & 100.00 \\
 & Portability $\uparrow$ & 36.58 & 37.00 & 34.73 & 59.28 & 61.02 \\
 & Locality $\uparrow$ & 30.40 & 29.28 & 34.80 & 41.54 & 46.39 \\
 & Fluency $\uparrow$ & 581.00 & 573.06 & 558.91 & 587.17 & 585.58 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 107.47 & 87.17 & 68.92 & 70.64 & 34.08 \\
\midrule
\multirow{5}{*}{\textbf{ZsRE}} & Edit Succ. $\uparrow$ & 96.66 & 95.61 & 43.60 & 100.00 & 100.00 \\
 & Portability $\uparrow$ & 52.90 & 52.73 & 43.90 & 54.47 & 55.52 \\
 & Locality $\uparrow$ & 26.61 & 24.79 & 51.38 & 53.84 & 56.97 \\
 & Fluency $\uparrow$ & 573.02 & 563.42 & 560.94 & 580.10 & 562.70 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 53.88 & 38.67 & 30.36 & 27.33 & 15.50 \\
\midrule
\multirow{4}{*}{\textbf{WikiBio}} & Edit Succ. $\uparrow$ & 95.83 & 94.54 & 59.41 & 100.00 & 99.88 \\
 & Locality $\uparrow$ & 68.38 & 69.96 & 28.94 & 35.34 & 70.60 \\
 & Fluency $\uparrow$ & 617.67 & 616.65 & 615.50 & 618.12 & 617.88 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 3.70 & 3.51 & 1.89 & 3.67 & 2.15 \\
\midrule
\multirow{5}{*}{\textbf{Wiki$_{cf}$}} & Edit Succ. $\uparrow$ & 98.68 & 98.13 & 36.13 & 100.00 & 100.00 \\
 & Portability $\uparrow$ & 42.45 & 44.16 & 29.37 & 72.39 & 73.49 \\
 & Locality $\uparrow$ & 21.13 & 19.48 & 38.37 & 40.76 & 45.88 \\
 & Fluency $\uparrow$ & 585.40 & 576.26 & 566.55 & 586.80 & 583.29 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 109.97 & 122.48 & 89.24 & 54.71 & \\
\bottomrule
\end{tabular}
}
\caption{Main results on all datasets of Llama2-7b-chat}
\label{tab:main_results_llama2}
\end{table}




\begin{table*}[ht]
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\textbf{DataSet} & \textbf{Metric} & \textbf{ROME} & \textbf{MEMIT} & \textbf{FT-L} & \textbf{FT-M} & \textbf{ICE} \\
\midrule
\multirow{5}{*}{\textbf{WikiData$_{recent}$}} 
 & Edit succ. $\uparrow$ & 99.24 & 78.31 & 63.99 & 100.00 & 100.00 \\
 & Portability $\uparrow$ & 30.74 & 24.97 & 29.03 & 36.74 & 35.76 \\
 & Locality $\uparrow$ & 25.37 & 32.73 & 61.45 & 61.07 & 63.45 \\
 & Fluency $\uparrow$ & 603.82 & 600.54 & 591.86 & 604.07 & 560.96 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 316.38 & 6.79 & 25.26 & 35.81 & 7.91 \\
\midrule
\multirow{5}{*}{\textbf{ZsRE}} 
 & Edit succ. $\uparrow$  & 99.88 & 67.39 & 64.25 & 100.00 & 99.92 \\
 & Portability $\uparrow$ & 41.99 & 41.45 & 42.51 & 48.41 & 46.84 \\
 & Locality $\uparrow$ & 67.83 & 80.84 & 32.18 & 31.39 & 34.44 \\
 & Fluency $\uparrow$ & 578.87 & 591.98 & 571.71 & 583.63 & 554.74 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 15.35 & 5.54 & 12.40 & 17.28 & 9.40 \\
\midrule
\multirow{4}{*}{\textbf{WikiBio}} 
 & Edit succ. $\uparrow$  & 81.52 & 57.31 & 51.59 & 100.00 & 100.00 \\
 & Locality $\uparrow$ & 27.49 & 39.65 & 66.66 & 63.87 & 63.67 \\
 & Fluency $\uparrow$ & 633.41 & 632.89 & 626.17 & 631.93 & 629.60 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 2.11 & 1.87 & 1.16 & 2.12 & 2.22 \\
\midrule
\multirow{5}{*}{\textbf{WikiData$_{counterfact}$}} 
 & Edit succ. $\uparrow$  & 96.08 & 55.03 & 40.85 & 100.00 & 100.00 \\
 & Portability $\uparrow$ & 31.31 & 20.00 & 20.09 & 42.08 & 39.78 \\
 & Locality $\uparrow$ & 16.67 & 24.79 & 65.29 & 63.43 & 67.06 \\
 & Fluency $\uparrow$ & 600.94 & 604.58 & 596.77 & 602.91 & 560.33 \\
 & $\text{PPL}_{r}$ $\downarrow$ & 3.71 & 11.10 & 26.55 & 12.64 & 8.05 \\
\bottomrule
\end{tabular}
}
\caption{Main results on all datasets of GPT2-XL}
\label{tab:main_results_gpt2}
\end{table*}





% \begin{table*}[ht]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccccccc}
% \toprule
% \textbf{DataSet} & \textbf{Metric} & \textbf{SERAC} & \textbf{ICE} & \textbf{AdaLoRA} & \textbf{MEND} & \textbf{ROME} & \textbf{MEMIT} & \textbf{FT-L} & \textbf{FT-M} \\
% \midrule
% \textbf{WikiData$_{recent}$} & Edit Succ. $\uparrow$ & 98.68 & 60.74 & 65.61 & 95.75 & 85.08 & 85.32 & 71.18 & 100.00 \\
%  & Portability $\uparrow$ & 63.52 & 36.93 & 47.22 & 55.88 & 37.45 & 37.94 & 48.71 & 64.86 \\
%  & Locality $\uparrow$ & 100.00 & 33.34 & 55.78 & 94.76 & 66.20 & 64.78 & 63.70 & 63.70 \\
%  & Fluency $\uparrow$ & 553.19 & 531.01 & 537.51 & 557.11 & 574.28 & 566.66 & 549.35 & 574.32 \\
% \midrule
% \textbf{ZsRE} & Edit Succ. $\uparrow$ & 99.67 & 66.01 & 69.86 & 96.74 & 96.57 & 83.07 & 54.65 & 99.87 \\
%  & Portability $\uparrow$ & 56.48 & 63.94 & 52.95 & 60.41 & 52.20 & 51.43 & 45.02 & 60.31 \\
%  & Locality $\uparrow$ & 30.23 & 23.14 & 72.21 & 92.79 & 27.14 & 25.46 & 71.12 & 89.78 \\
%  & Fluency $\uparrow$ & 410.89 & 541.14 & 532.82 & 524.33 & 570.47 & 559.72 & 474.18 & 552.26 \\
% \midrule
% \textbf{WikiBio} & Edit Succ. $\uparrow$ & 99.69 & 95.53 & 97.02 & 93.66 & 95.05 & 94.29 & 66.27 & 100.00 \\
%  & Locality $\uparrow$ & 69.79 & 47.90 & 57.87 & 69.51 & 46.96 & 51.56 & 60.14 & 93.38 \\
%  & Fluency $\uparrow$ & 606.95 & 632.92 & 615.86 & 609.39 & 617.25 & 616.65 & 604.00 & 612.69 \\
% \midrule
% \textbf{WikiData$_{counterfact}$} & Edit Succ. $\uparrow$ & 99.99 & 69.83 & 72.14 & 80.03 & 83.21 & 83.41 & 51.12 & 100.00 \\
%  & Portability $\uparrow$ & 76.07 & 45.32 & 55.17 & 52.01 & 38.69 & 40.09 & 39.07 & 69.68 \\
%  & Locality $\uparrow$ & 98.96 & 32.38 & 66.78 & 94.38 & 65.40 & 63.68 & 62.51 & 74.20 \\
%  & Fluency $\uparrow$ & 549.91 & 547.22 & 553.85 & 555.72 & 578.84 & 568.58 & 544.80 & 575.62 \\
% \midrule
% \textbf{ConvSent} & Edit Succ. $\uparrow$ & 62.75 & 52.78 & 44.89 & 50.76 & 45.79 & 44.75 & 49.50 & 46.10 \\
%  & Locality $\downarrow$ & 0.26 & 49.73 & 0.18 & 3.42 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & Fluency $\uparrow$ & 458.21 & 621.45 & 606.42 & 379.43 & 606.32 & 602.62 & 607.86 & 592.52 \\
% \midrule
% \textbf{Sanitation} & Edit Succ. $\uparrow$ & 0.00 & 72.50 & 2.50 & 0.00 & 85.00 & 48.75 & 0.00 & 75.00 \\
%  & Locality $\uparrow$ & 100.00 & 56.58 & 65.50 & 5.29 & 50.31 & 67.47 & 14.78 & 47.07 \\
%  & Fluency $\uparrow$ & 416.29 & 794.15 & 330.44 & 407.18 & 465.12 & 466.10 & 439.10 & 416.29 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Main results on all datasets of Llama2 (see Table 4 in the survey).}
% \label{tab:main_results_llama2}
% \end{table*}

